Differential Equation Based Wall Distance Approaches for Maritime Engineering Flows

The paper is concerned with modeling and simulating approaches of wall distance functions based on Partial Differential Equations (PDE). The distance to the nearest wall is required for many industrial problems in Computational Fluid Dynamics (CFD). The first part of the manuscript addresses fundamental aspects of wall distance modeling and simulation. The following approaches are considered: Nonlinear and linear p-Poisson and Screened-Poisson methods, Eikonal and regularized Eikonal or Hamilton-Jacobi methods, and alternatives using Laplace equations. Following the definition of boundary and initial conditions, the discrete approximation and relevant measures to increase its numerical robustness are described. In the second part, the different methods are applied to hydrodynamic and aerodynamic flow applications from maritime engineering, each relying on Shear Stress Transport (SST) strategies for turbulence modeling that require the distance to the nearest wall at different procedural points. The hydrodynamic behavior of a model scale bulk carrier cruising at ReL=7.246E+6 and Fn = 0.142 is investigated on the influence of the wall distance formulation for predicting resistance and propulsion behavior in conjunction with statistical turbulence modeling method. It is shown that the different wall distance modeling barely influences relevant integral hydrodynamic quantities such as drag, trim, and sinkage, and related errors are in the range of O(0.1%) and, therefore, significantly below typical modeling, discretization, and approximation errors. Subsequently, the wall distance methods were investigated for the aerodynamic analysis of a full-scale feeder ship at ReL = 5E+08. A hybrid averaged/filtered approach, in line with the Improved Delayed Detached Eddy Simulation (IDDES) model, is utilized, and the results indicate an improved sensitivity to the choice of the wall distance model.

==> tex/playground.tex <==
\subsection{Laplacian-Iterations}

\begin{alignat}{2}
    \frac{\partial^2 d}{\partial x_k^2} \bigg|_{i+1} &= \frac{\partial}{\partial x_k} \left[ \frac{\partial d}{\partial x_k} \bigg/ \bigg| \frac{\partial d}{\partial x_k} \bigg| \right] \bigg|_{i} \qquad &&\text{in} \qquad \Omega \label{equ:iterative_laplacian} \, , \\
    d \bigg|_{i+1} &= 0 \qquad &&\text{on} \qquad \Gamma^\text{wall} \, , \\
    \frac{\partial d}{\partial n} \bigg|_{i+1} &= 0 \qquad &&\text{on} \qquad \Gamma^\text{symm} \, , \\
    \frac{\partial d}{\partial n} \bigg|_{i+1} &= 1 \qquad &&\text{on} \qquad \Gamma^\text{rest} \, ,
\end{alignat}

Convergence acceleration via definition of optimization (minimization) problem
\begin{align}
    J = \int \left( |p_k| - 1 \right)^2 \mathrm{d} \Omega
    \qquad \qquad \text{with} \qquad \qquad
    p_k = \frac{\partial d}{\partial x_k} \label{equ:objective}
\end{align}

Definition of augmented cost functional aka Lagrangian
\begin{align}
    L = J + \int \hat{p}_k \left( p_k - \frac{\partial d}{\partial x_k} \right) + \frac{r}{2} \left( p_k - \frac{\partial d}{\partial x_k} \right)^2 \mathrm{d} \Omega \label{equ:lagrangian}
\end{align}
where $\hat{p}_k$ and $r>0$ refer to a Lagrangian multiplier and a penalty term, respectively. Combining \ref{equ:objective} and \ref{equ:lagrangian} provides
\begin{align}
    L = \int \left( |p_k| - 1 \right)^2 + \hat{p}_k \left( p_k - \frac{\partial d}{\partial x_k} \right) + \frac{r}{2} \left( p_k - \frac{\partial d}{\partial x_k} \right)^2 \mathrm{d} \Omega
\end{align}
A total variation yields
\begin{align}
    %L^\prime &= \int 2 \left( |p_k| - 1 \right) |p_k|^\prime + \hat{p}_k \left( p_k^\prime - \frac{\partial d^\prime}{\partial x_k} \right) + r \left( p_k - \frac{\partial d}{\partial x_k} \right) \left(p_k^\prime - \frac{\partial d^\prime}{\partial x_k} \right) \mathrm{d} \Omega \\
    L^\prime &= \int 
    2 \left( |p_k| - 1 \right) |p_k|^\prime 
    + p_k^\prime \left[ \hat{p}_k + r \left( p_k - \frac{\partial d}{\partial x_k} \right) \right] 
    - \frac{\partial d^\prime}{\partial x_k} \left[ \hat{p}_k + r \left( p_k - \frac{\partial d}{\partial x_k} \right) \right]
    + \hat{p}^\prime \left[ p_k - \frac{\partial d}{\partial x_k} \right]
    \mathrm{d} \Omega \label{equ:varied_lagrangian} \, .
\end{align}

Optimality conditions provide
\begin{align}
    \hat{p}_k = r \left( \frac{\partial d}{\partial x_k} - p_k \right)
\end{align}
as well as
\begin{align}
    \int \frac{\partial d^\prime}{\partial x_k} \left[ \hat{p}_k + r \left( p_k - \frac{\partial d}{\partial x_k} \right) \right] \mathrm{d} \Omega
    =
    \int d^\prime  \left[ \hat{p}_k + r \left( p_k - \frac{\partial d}{\partial x_k} \right) \right] n_k \mathrm{d} \Gamma
    - \int d^\prime \frac{\partial}{\partial x_k} \left[ \hat{p}_k + r \left( p_k - \frac{\partial d}{\partial x_k} \right) \right] \mathrm{d} \Omega
\end{align}
and thus
\begin{alignat}{2}
    r \frac{\partial^2 d}{\partial x_k^2} &= \frac{\partial \hat{p}_k}{\partial x_k} + r \frac{\partial p_k}{\partial x_k} \qquad &&\text{in} \qquad \Omega \label{equ:admm} \, , \\
    TBA &= 0 \qquad &&\text{on} \qquad \Gamma^\text{wall} \, , \\
    \left[ \hat{p}_k + r \left( p_k - \frac{\partial d}{\partial x_k} \right) \right] n_k &= 0 \qquad &&\text{on} \qquad \Gamma^\text{symm} \, , \\
    \left[ \hat{p}_k + r \left( p_k - \frac{\partial d}{\partial x_k} \right) \right] n_k &= 0 \qquad &&\text{on} \qquad \Gamma^\text{rest} \, ,
\end{alignat}



%Some crucial aspects for the approximation are: a) The connecting vector $d_i^F$ between two face adjacent cell centers does not necessarily pierce through the face center F and sometimes does not even pierce through the face at all, b) the connecting vector $d_\mathrm{i}^\mathrm{* F}$ is not necessarily co-linear to the face normal $n_\mathrm{i}$ and c) faces are not necessarily centered between the center of the neighboring cell.

%Local approximations are constructed from values extracted at the cell center $P \in [1, NP]$, the face centers $F \in [1, NF]$ separating the control volume around P from the neighboring control volumes and the centers of the boundary control volume denoted by $B \in [1, NB]$. Here, NF denotes the number of faces and neighbors per cell, viz. $\mathrm{F}(\mathrm{P}) = \left[1, ..., \mathrm{NF} \right]$ as well as $\mathrm{NB}(\mathrm{P}) = \left[1, ..., \mathrm{NB} \right]$. Fig. \ref{fig:finite_volume_approximation} (a) shows an arbitrary arrangement of two adjacent polyhedral control volumes that share the connecting vector between P and NB(P) through F(P), viz.
%They employ the cell size $\Delta \Omega^\mathrm{* P}$ as well as the area $\Delta \Gamma^\mathrm{* F}$ and the respective area vector $\Delta \Gamma_\mathrm{i}^\mathrm{* F} = \Delta \Gamma^\mathrm{* F} \, n_\mathrm{i}$ of all cell adjacent faces where $n_\mathrm{i}$ represents the local face normal.
